Unsupervised Anomaly Detection in Medical Images Using Masked Diffusion Model

It can be challenging to identify brain MRI anomalies using supervised deep-learning techniques due to anatomical heterogeneity and the requirement for pixel-level labeling. Unsupervised anomaly detection approaches provide an alternative solution by relying only on sample-level labels of healthy brains to generate a desired representation to identify abnormalities at the pixel level. Although, generative models are crucial for generating such anatomically consistent representations of healthy brains, accurately generating the intricate anatomy of the human brain remains a challenge. In this study, we present a method called masked-DDPM (mDPPM), which introduces masking-based regularization to reframe the generation task of diffusion models. Specifically, we introduce Masked Image Modeling (MIM) and Masked Frequency Modeling (MFM) in our self-supervised approach that enables models to learn visual representations from unlabeled data. To the best of our knowledge, this is the first attempt to apply MFM in DPPM models for medical applications. We evaluate our approach on datasets containing tumors and numerous sclerosis lesions and exhibit the superior performance of our unsupervised method as compared to the existing fully/weakly supervised baselines. Code is available at https://github.com/hasan1292/mDDPM.

==> template/references.tex <==
@article{vernooij2007incidental,
  title={Incidental findings on brain MRI in the general population},
  author={Vernooij, Meike W and Ikram, M Arfan and Tanghe, Herv{\'e} L and Vincent, Arnaud JPE and Hofman, Albert and Krestin, Gabriel P and Niessen, Wiro J and Breteler, Monique MB and van der Lugt, Aad},
  journal={New England Journal of Medicine},
  volume={357},
  number={18},
  pages={1821--1828},
  year={2007},
  publisher={Mass Medical Soc}
}
@article{dice1945measures,
  title={Measures of the amount of ecologic association between species},
  author={Dice, Lee R},
  journal={Ecology},
  volume={26},
  number={3},
  pages={297--302},
  year={1945},
  publisher={JSTOR}
}
@inproceedings{davis2006relationship,
  title={The relationship between Precision-Recall and ROC curves},
  author={Davis, Jesse and Goadrich, Mark},
  booktitle={Proceedings of the 23rd international conference on Machine learning},
  pages={233--240},
  year={2006}
}
@misc{wang2023fremae,
      title={FreMAE: Fourier Transform Meets Masked Autoencoders for Medical Image Segmentation}, 
      author={Wenxuan Wang and Jing Wang and Chen Chen and Jianbo Jiao and Lichao Sun and Yuanxiu Cai and Shanshan Song and Jiangyun Li},
      year={2023},
      eprint={2304.10864},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@misc{gao2022convmae,
      title={ConvMAE: Masked Convolution Meets Masked Autoencoders}, 
      author={Peng Gao and Teli Ma and Hongsheng Li and Ziyi Lin and Jifeng Dai and Yu Qiao},
      year={2022},
      eprint={2205.03892},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@misc{he2021masked,
      title={Masked Autoencoders Are Scalable Vision Learners}, 
      author={Kaiming He and Xinlei Chen and Saining Xie and Yanghao Li and Piotr Dollár and Ross Girshick},
      year={2021},
      eprint={2111.06377},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@misc{ixii,   
   
    url = {https://brain-development.org/ixi-dataset/},   
    
       
}
@book{nussbaumer1981fast,
  title={The fast Fourier transform},
  author={Nussbaumer, Henri J and Nussbaumer, Henri J},
  year={1981},
  publisher={Springer}
}
@inproceedings{chen2019drop,
  title={Drop an octave: Reducing spatial redundancy in convolutional neural networks with octave convolution},
  author={Chen, Yunpeng and Fan, Haoqi and Xu, Bing and Yan, Zhicheng and Kalantidis, Yannis and Rohrbach, Marcus and Yan, Shuicheng and Feng, Jiashi},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={3435--3444},
  year={2019}
}
@article{kauffmann2014neural,
  title={The neural bases of spatial frequency processing during scene perception},
  author={Kauffmann, Louise and Ramano{\"e}l, Stephen and Peyrin, Carole},
  journal={Frontiers in integrative neuroscience},
  volume={8},
  pages={37},
  year={2014},
  publisher={Frontiers Media SA}
}
@article{10.1145/3464423,
author = {Fernando, Tharindu and Gammulle, Harshala and Denman, Simon and Sridharan, Sridha and Fookes, Clinton},
title = {Deep Learning for Medical Anomaly Detection – A Survey},
year = {2021},
issue_date = {September 2022},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {54},
number = {7},
issn = {0360-0300},
url = {https://doi.org/10.1145/3464423},
doi = {10.1145/3464423},
abstract = {Machine learning–based medical anomaly detection is an important problem that has been extensively studied. Numerous approaches have been proposed across various medical application domains and we observe several similarities across these distinct applications. Despite this comparability, we observe a lack of structured organisation of these diverse research applications such that their advantages and limitations can be studied. The principal aim of this survey is to provide a thorough theoretical analysis of popular deep learning techniques in medical anomaly detection. In particular, we contribute a coherent and systematic review of state-of-the-art techniques, comparing and contrasting their architectural differences as well as training algorithms. Furthermore, we provide a comprehensive overview of deep model interpretation strategies that can be used to interpret model decisions. In addition, we outline the key limitations of existing deep medical anomaly detection techniques and propose key research directions for further investigation.},
journal = {ACM Comput. Surv.},
month = {jul},
articleno = {141},
numpages = {37},
keywords = {machine learning, anomaly detection, Deep learning, temporal analysis}
}
@article{bruno2015understanding,
  title={Understanding and confronting our mistakes: the epidemiology of error in radiology and strategies for error reduction},
  author={Bruno, Michael A and Walker, Eric A and Abujudeh, Hani H},
  journal={Radiographics},
  volume={35},
  number={6},
  pages={1668--1676},
  year={2015},
  publisher={Radiological Society of North America}
}

@article{Drew.2013,
 author = {Drew, Trafton and V{\~o}, Melissa L-H and Wolfe, Jeremy M.},
 year = {2013},
 title = {{The invisible gorilla strikes again: sustained inattentional blindness in expert observers}},
 pages = {1848--1853},
 volume = {24},
 number = {9},
 journal = {{Psychological science}},
 abstract = {Researchers have shown that people often miss the occurrence of an unexpected yet salient event if they are engaged in a different task, a phenomenon known as inattentional blindness. However, demonstrations of inattentional blindness have typically involved naive observers engaged in an unfamiliar task. What about expert searchers who have spent years honing their ability to detect small abnormalities in specific types of images? We asked 24 radiologists to perform a familiar lung-nodule detection task. A gorilla, 48 times the size of the average nodule, was inserted in the last case that was presented. Eighty-three percent of the radiologists did not see the gorilla. Eye tracking revealed that the majority of those who missed the gorilla looked directly at its location. Thus, even expert searchers, operating in their domain of expertise, are vulnerable to inattentional blindness.}
}

@article{Lundervold.2019,
 author = {Lundervold, Alexander Selvikv{\aa}g and Lundervold, Arvid},
 year = {2019},
 title = {{An overview of deep learning in medical imaging focusing on MRI}},
 pages = {102--127},
 volume = {29},
 number = {2},
 journal = {{Zeitschrift fur medizinische Physik}},
 abstract = {What has happened in machine learning lately, and what does it mean for the future of medical image analysis? Machine learning has witnessed a tremendous amount of attention over the last few years. The current boom started around 2009 when so-called deep artificial neural networks began outperforming other established models on a number of important benchmarks. Deep neural networks are now the state-of-the-art machine learning models across a variety of areas, from image analysis to natural language processing, and widely deployed in academia and industry. These developments have a huge potential for medical imaging technology, medical data analysis, medical diagnostics and healthcare in general, slowly being realized. We provide a short overview of recent advances and some associated challenges in machine learning applied to medical image processing and image analysis. As this has become a very broad and fast expanding field we will not survey the entire landscape of applications, but put particular focus on deep learning in MRI. Our aim is threefold: (i) give a brief introduction to deep learning with pointers to core references; (ii) indicate how deep learning has been applied to the entire MRI processing chain, from acquisition to image retrieval, from segmentation to disease prediction; (iii) provide a starting point for people interested in experimenting and perhaps contributing to the field of deep learning for medical imaging by pointing out good educational resources, state-of-the-art open-source code, and interesting sources of data and problems related medical imaging.}
}


 @article{Kim.2014,
author = {Kim, Young W. and Mansfield, Liem T.},
title = {Fool Me Twice: Delayed Diagnoses in Radiology With Emphasis on Perpetuated Errors},
journal = {American Journal of Roentgenology},
volume = {202},
number = {3},
pages = {465-470},
year = {2014},
doi = {10.2214/AJR.13.11493 },
    note ={PMID: 24555582 },

URL = { 
        https://doi.org/10.2214/AJR.13.11493
    
},
eprint = { 
        https://doi.org/10.2214/AJR.13.11493
    
}

}

@inproceedings{shortagerad,
author = {Mirza, Kashif and Vinayak, Sudhir and Khan, Tanveer and Shituma, Shikuku and Mugoma, Godfred},
year = {2012},
month = {11},
pages = {},
booktitle  = {Radiological Society of North America 2012 Scientific Assembly and Annual Meeting},
title = {Overcoming Shortage of Radiologists by Implementing a Cross-Border PACS, RIS and HIS in East Africa (EA) (Kenya, Uganda and Tanzania)}
}

@article{shen2017deep,
  title={Deep learning in medical image analysis},
  author={Shen, Dinggang and Wu, Guorong and Suk, Heung-Il},
  journal={Annual review of biomedical engineering},
  volume={19},
  pages={221},
  year={2017},
  publisher={NIH Public Access}
}

@article{ELLIS2022100068,
title = {Twelve key challenges in medical machine learning and solutions},
journal = {Intelligence-Based Medicine},
volume = {6},
pages = {100068},
year = {2022},
issn = {2666-5212},
author = {Randall J. Ellis and Ryan M. Sander and Alfonso Limon},
keywords = {Machine learning, Baseline models, Performance metrics, Imbalanced datasets, Model and label uncertainty, Reproducibility},
abstract = {The utility of machine learning in biomedicine is being investigated in various contexts, including for diagnostic and interpretive purposes for imaging modalities, quantifying disease risk, and processing text from physician and patient reports. To best facilitate the potential of machine learning, clinicians and computational scientists must inform one another about the nature of their clinical challenges and available methods for solving them, respectively. To this end, clinicians need to critically evaluate machine learning studies conducted to solve relevant problems in medicine. This article serves as a checklist for clinicians to understand and appraise machine learning studies and help facilitate productive conversations between the clinical and data science communities to improve human health.}
}

@article{karimi2020deep,
  title={Deep learning with noisy labels: Exploring techniques and remedies in medical image analysis},
  author={Karimi, Davood and Dou, Haoran and Warfield, Simon K and Gholipour, Ali},
  journal={Medical Image Analysis},
  volume={65},
  pages={101759},
  year={2020},
  publisher={Elsevier}
}

@article{Johnson.2019,
 author = {Johnson, Justin M. and Khoshgoftaar, Taghi M.},
 year = {2019},
 title = {{Survey on deep learning with class imbalance}},
 pages = {1--54},
 volume = {6},
 number = {1},
 journal = {{Journal of Big Data}},
 abstract = {The purpose of this study is to examine existing deep learning techniques for addressing class imbalanced data. Effective classification with imbalanced data is an important area of research, as high class imbalance is naturally inherent in many real-world applications, e.g., fraud detection and cancer detection. Moreover, highly imbalanced data poses added difficulty, as most learners will exhibit bias towards the majority class, and in extreme cases, may ignore the minority class altogether. Class imbalance has been studied thoroughly over the last two decades using traditional machine learning models, i.e. non-deep learning. Despite recent advances in deep learning, along with its increasing popularity, very little empirical work in the area of deep learning with class imbalance exists. Having achieved record-breaking performance results in several complex domains, investigating the use of deep neural networks for problems containing high levels of class imbalance is of great interest. Available studies regarding class imbalance and deep learning are surveyed in order to better understand the efficacy of deep learning when applied to class imbalanced data. This survey discusses the implementation details and experimental results for each study, and offers additional insight into their strengths and weaknesses. Several areas of focus include: data complexity, architectures tested, performance interpretation, ease of use, big data application, and generalization to other domains. We have found that research in this area is very limited, that most existing work focuses on computer vision tasks with convolutional neural networks, and that the effects of big data are rarely considered. Several traditional methods for class imbalance, e.g. data sampling and cost-sensitive learning, prove to be applicable in deep learning, while more advanced methods that exploit neural network feature learning abilities show promising results. The survey concludes with a discussion that highlights various gaps in deep learning from class imbalanced data for the purpose of guiding future research.}
}

@article{baur2021autoencoders,
  title={Autoencoders for unsupervised anomaly segmentation in brain MR images: a comparative study},
  author={Baur, Christoph and Denner, Stefan and Wiestler, Benedikt and Navab, Nassir and Albarqouni, Shadi},
  journal={Medical Image Analysis},
  pages={101952},
  year={2021},
  publisher={Elsevier}
}


@inproceedings{Chen.2018,
 author = {Chen, Xiaoran and Konukoglu, Ender},
 title = {{Unsupervised Detection of Lesions in Brain MRI using Constrained Adversarial Auto-encoders}},
 publisher = {PMLR},
 series = {{Proceedings of Machine Learning Research}},
 booktitle = {{International Conference on Medical Imaging with Deep Learning (MIDL)}},
 year = {2018}
}

@article{chen2020unsupervised,
  title={Unsupervised lesion detection via image restoration with a normative prior},
  author={Chen, Xiaoran and You, Suhang and Tezcan, Kerem Can and Konukoglu, Ender},
  journal={Medical image analysis},
  volume={64},
  pages={101713},
  year={2020},
  publisher={Elsevier}
}
@article{Schlegl.2019,
 author = {Schlegl, Thomas and Seeb{\"o}ck, Philipp and Waldstein, Sebastian M. and Langs, Georg and Schmidt-Erfurth, Ursula},
 year = {2019},
 title = {{f-AnoGAN: Fast unsupervised anomaly detection with generative adversarial networks}},
 pages = {30--44},
 volume = {54},
 journal = {{Medical image analysis}},
 abstract = {Obtaining expert labels in clinical imaging is difficult since exhaustive annotation is time-consuming. Furthermore, not all possibly relevant markers may be known and sufficiently well described a priori to even guide annotation. While supervised learning yields good results if expert labeled training data is available, the visual variability, and thus the vocabulary of findings, we can detect and exploit, is limited to the annotated lesions. Here, we present fast AnoGAN (f-AnoGAN), a generative adversarial network (GAN) based unsupervised learning approach capable of identifying anomalous images and image segments, that can serve as imaging biomarker candidates. We build a generative model of healthy training data, and propose and evaluate a fast mapping technique of new data to the GAN's latent space. The mapping is based on a trained encoder, and anomalies are detected via a combined anomaly score based on the building blocks of the trained model - comprising a discriminator feature residual error and an image reconstruction error. In the experiments on optical coherence tomography data, we compare the proposed method with alternative approaches, and provide comprehensive empirical evidence that f-AnoGAN outperforms alternative approaches and yields high anomaly detection accuracy. In addition, a visual Turing test with two retina experts showed that the generated images are indistinguishable from real normal retinal OCT images. The f-AnoGAN code is available at https://github.com/tSchlegl/f-AnoGAN.}
}


@article{wolleb2022diffusion,
  title={Diffusion Models for Medical Anomaly Detection},
  author={Wolleb, Julia and Bieder, Florentin and Sandk{\"u}hler, Robin and Cattin, Philippe C},
  journal={arXiv preprint arXiv:2203.04306   } ,
  year={2022}
}

@inproceedings{wyatt2022anoddpm,
  title={AnoDDPM: Anomaly Detection With Denoising Diffusion Probabilistic Models Using Simplex Noise},
  author={Wyatt, Julian and Leach, Adam and Schmon, Sebastian M and Willcocks, Chris G},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={650--656},
  year={2022}
}

@article{pinaya2022fast,
  title={Fast Unsupervised Brain Anomaly Detection and Segmentation with Diffusion Models},
  author={Pinaya, Walter HL and Graham, Mark S and Gray, Robert and Da Costa, Pedro F and Tudosiu, Petru-Daniel and Wright, Paul and Mah, Yee H and MacKinnon, Andrew D and Teo, James T and Jager, Rolf and others},
  journal={arXiv preprint arXiv:2206.03461  } ,
  year={2022}
}

@inproceedings{sanchez2022healthy,
  title={What is healthy? generative counterfactual diffusion for lesion localization},
  author={Sanchez, Pedro and Kascenas, Antanas and Liu, Xiao and O’Neil, Alison Q and Tsaftaris, Sotirios A},
  booktitle={MICCAI Workshop on Deep Generative Models},
  pages={34--44},
  year={2022},
  organization={Springer}
}

@article{ho2020denoising,
  title={Denoising diffusion probabilistic models},
  author={Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={6840--6851},
  year={2020}
}

@article{dhariwal2021diffusion,
  title={Diffusion models beat gans on image synthesis},
  author={Dhariwal, Prafulla and Nichol, Alexander},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={8780--8794},
  year={2021}
}
@inproceedings{rombach2022high,
  title={High-resolution image synthesis with latent diffusion models},
  author={Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Bj{\"o}rn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10684--10695},
  year={2022}
}

@inproceedings{kascenas2021denoising,
  title={Denoising Autoencoders for Unsupervised Anomaly Detection in Brain MRI},
  author={Kascenas, Antanas and Pugeault, Nicolas and O'Neil, Alison Q},
 publisher = {PMLR},
 series = {{Proceedings of Machine Learning Research}},
 booktitle = {{International Conference on Medical Imaging with Deep Learning (MIDL)}},
  year={2022}
}

@article{tschuchnig2022anomaly,
  title={Anomaly Detection in Medical Imaging-A Mini Review},
  author={Tschuchnig, Maximilian E and Gadermayr, Michael},
  journal={Data Science--Analytics and Applications},
  pages={33--38},
  year={2022},
  publisher={Springer}
}
@inproceedings{baur2018deep,
  title={Deep autoencoding models for unsupervised anomaly segmentation in brain MR images},
  author={Baur, Christoph and Wiestler, Benedikt and Albarqouni, Shadi and Navab, Nassir},
  booktitle={International MICCAI brainlesion workshop},
  pages={161--169},
  year={2018},
  organization={Springer}
}

@inproceedings{baur2020scale,
  title={Scale-space autoencoders for unsupervised anomaly segmentation in brain mri},
  author={Baur, Christoph and Wiestler, Benedikt and Albarqouni, Shadi and Navab, Nassir},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={552--561},
  year={2020},
  organization={Springer}
}

@inproceedings{baur2020bayesian,
  title={Bayesian skip-autoencoders for unsupervised hyperintense anomaly detection in high resolution brain MRI},
  author={Baur, Christoph and Wiestler, Benedikt and Albarqouni, Shadi and Navab, Nassir},
  booktitle={2020 IEEE 17th International Symposium on Biomedical Imaging (ISBI)},
  pages={1905--1909},
  year={2020},
  organization={IEEE}
}


@inproceedings{zimmerer2018context,
  title={Context-encoding Variational Autoencoder for Unsupervised Anomaly Detection},
  author={Zimmerer, David and Kohl, Simon and Petersen, Jens and Isensee, Fabian and Maier-Hein, Klaus},
  booktitle={International Conference on Medical Imaging with Deep Learning--Extended Abstract Track},
  year={2019}
}
@article{bengs2021three,
  title={Three-dimensional deep learning with spatial erasing for unsupervised anomaly segmentation in brain MRI},
  author={Bengs, Marcel and Behrendt, Finn and Kr{\"u}ger, Julia and Opfer, Roland and Schlaefer, Alexander},
  journal={International journal of computer assisted radiology and surgery},
  volume={16},
  number={9},
  pages={1413--1423},
  year={2021},
  publisher={Springer}
}

@article{pinaya2022unsupervised,
  title={Unsupervised brain imaging 3D anomaly detection and segmentation with transformers},
  author={Pinaya, Walter HL and Tudosiu, Petru-Daniel and Gray, Robert and Rees, Geraint and Nachev, Parashkev and Ourselin, Sebastien and Cardoso, M Jorge},
  journal={Medical Image Analysis},
  volume={79},
  pages={102475},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{behrendt2022capturing,
  title={Capturing Inter-Slice Dependencies of 3D Brain MRI-Scans for Unsupervised Anomaly Detection},
  author={Behrendt, Finn and Bengs, Marcel and Bhattacharya, Debayan and Kr{\"u}ger, Julia and Opfer, Roland and Schlaefer, Alexander},
  booktitle={Medical Imaging with Deep Learning},
  year={2022}
}

@article{SILVARODRIGUEZ2022102526,
title = {Constrained unsupervised anomaly segmentation},
journal = {Medical Image Analysis},
volume = {80},
pages = {102526},
year = {2022},
author = {Julio Silva-Rodríguez and Valery Naranjo and Jose Dolz},
keywords = {Unsupervised anomaly localization, Constraint segmentation, Brain lesions},
abstract = {Current unsupervised anomaly localization approaches rely on generative models to learn the distribution of normal images, which is later used to identify potential anomalous regions derived from errors on the reconstructed images. To address the limitations of residual-based anomaly localization, very recent literature has focused on attention maps, by integrating supervision on them in the form of homogenization constraints. In this work, we propose a novel formulation that addresses the problem in a more principled manner, leveraging well-known knowledge in constrained optimization. In particular, the equality constraint on the attention maps in prior work is replaced by an inequality constraint, which allows more flexibility. In addition, to address the limitations of penalty-based functions we employ an extension of the popular log-barrier methods to handle the constraint. Last, we propose an alternative regularization term that maximizes the Shannon entropy of the attention maps, reducing the amount of hyperparameters of the proposed model. Comprehensive experiments on two publicly available datasets on brain lesion segmentation demonstrate that the proposed approach substantially outperforms relevant literature, establishing new state-of-the-art results for unsupervised lesion segmentation.}
}

@INPROCEEDINGS{8852144,

  author={Sato, Kazuki and Hama, Kenta and Matsubara, Takashi and Uehara, Kuniaki},

  booktitle={2019 International Joint Conference on Neural Networks (IJCNN)}, 

  title={Predictable Uncertainty-Aware Unsupervised Deep Anomaly Segmentation}, 

  year={2019},

  volume={},

  number={},

  pages={1-7},

  doi={10.1109/IJCNN.2019.8852144  }}


@inproceedings{meissen2022challenging,
  title={Challenging current semi-supervised anomaly segmentation methods for brain MRI},
  author={Meissen, Felix and Kaissis, Georgios and Rueckert, Daniel},
  booktitle={International MICCAI brainlesion workshop},
  pages={63--74},
  year={2022},
  organization={Springer}
}

@article{elfwing2018sigmoid,
  title={Sigmoid-weighted linear units for neural network function approximation in reinforcement learning},
  author={Elfwing, Stefan and Uchibe, Eiji and Doya, Kenji},
  journal={Neural Networks},
  volume={107},
  pages={3--11},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{perez2018film,
  title={Film: Visual reasoning with a general conditioning layer},
  author={Perez, Ethan and Strub, Florian and De Vries, Harm and Dumoulin, Vincent and Courville, Aaron},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  year={2018}
}

@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={International Conference on Medical image computing and computer-assisted intervention},
  pages={234--241},
  year={2015},
  organization={Springer}
}

@article{isensee2019automated,
  title={Automated brain extraction of multisequence MRI using artificial neural networks},
  author={Isensee, Fabian and Schell, Marianne and Pflueger, Irada and Brugnara, Gianluca and Bonekamp, David and Neuberger, Ulf and Wick, Antje and Schlemmer, Heinz-Peter and Heiland, Sabine and Wick, Wolfgang and others},
  journal={Human brain mapping},
  volume={40},
  number={17},
  pages={4952--4964},
  year={2019},
  publisher={Wiley Online Library}
}

@inproceedings{nguyen2021unsupervised,
  title={Unsupervised region-based anomaly detection in brain MRI with adversarial image inpainting},
  author={Nguyen, Bao and Feldman, Adam and Bethapudi, Sarath and Jennings, Andrew and Willcocks, Chris G},
  booktitle={2021 IEEE 18th international symposium on biomedical imaging (ISBI)},
  pages={1127--1131},
  year={2021},
  organization={IEEE}
}

@article{kawamoto2005improving,
  title={Improving clinical practice using clinical decision support systems: a systematic review of trials to identify features critical to success},
  author={Kawamoto, Kensaku and Houlihan, Caitlin A and Balas, E Andrew and Lobach, David F},
  journal={Bmj},
  volume={330},
  number={7494},
  pages={765},
  year={2005},
  publisher={British Medical Journal Publishing Group}
}

@article{lesjak2018novel,
  title={A novel public MR image dataset of multiple sclerosis patients with lesion segmentations based on multi-rater consensus},
  author={Lesjak, {\v{Z}}iga and Galimzianova, Alfiia and Koren, Ale{\v{s}} and Lukin, Matej and Pernu{\v{s}}, Franjo and Likar, Bo{\v{s}}tjan and {\v{S}}piclin, {\v{Z}}iga},
  journal={Neuroinformatics},
  volume={16},
  number={1},
  pages={51--63},
  year={2018},
  publisher={Springer}
}

@article{baid2021rsna,
  title={The rsna-asnr-miccai brats 2021 benchmark on brain tumor segmentation and radiogenomic classification},
  author={Baid, Ujjwal and Ghodasara, Satyam and Mohan, Suyash and Bilello, Michel and Calabrese, Evan and Colak, Errol and Farahani, Keyvan and Kalpathy-Cramer, Jayashree and Kitamura, Felipe C and Pati, Sarthak and others},
  journal={arXiv preprint arXiv:2107.02314  } ,
  year={2021}
}

@article{bakas2017advancing,
  title={Advancing the cancer genome atlas glioma MRI collections with expert segmentation labels and radiomic features},
  author={Bakas, Spyridon and Akbari, Hamed and Sotiras, Aristeidis and Bilello, Michel and Rozycki, Martin and Kirby, Justin S and Freymann, John B and Farahani, Keyvan and Davatzikos, Christos},
  journal={Scientific data},
  volume={4},
  number={1},
  pages={1--13},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{menze2014multimodal,
  title={The multimodal brain tumor image segmentation benchmark (BRATS)},
  author={Menze, Bjoern H and Jakab, Andras and Bauer, Stefan and Kalpathy-Cramer, Jayashree and Farahani, Keyvan and Kirby, Justin and Burren, Yuliya and Porz, Nicole and Slotboom, Johannes and Wiest, Roland and others},
  journal={IEEE transactions on medical imaging},
  volume={34},
  number={10},
  pages={1993--2024},
  year={2014},
  publisher={IEEE}
}
@article{rohlfing2010sri24,
  title={The SRI24 multichannel atlas of normal adult human brain structure},
  author={Rohlfing, Torsten and Zahr, Natalie M and Sullivan, Edith V and Pfefferbaum, Adolf},
  journal={Human brain mapping},
  volume={31},
  number={5},
  pages={798--819},
  year={2010},
  publisher={Wiley Online Library}
}

@article{graham2022denoising,
  title={Denoising Diffusion Models for Out-of-Distribution Detection},
  author={Graham, Mark S and Pinaya, Walter HL and Tudosiu, Petru-Daniel and Nachev, Parashkev and Ourselin, Sebastien and Cardoso, M Jorge},
  journal={arXiv preprint arXiv:2211.07740},
  year={2022}
}

@article{raschkas_2018_mlxtend,
  author       = {Sebastian Raschka},
  title        = {MLxtend: Providing machine learning and data science 
                  utilities and extensions to Python’s  
                  scientific computing stack},
  journal      = {The Journal of Open Source Software},
  volume       = {3},
  number       = {24},
  month        = apr,
  year         = 2018,
  publisher    = {The Open Journal},
  doi          = {10.21105/joss.00638},
  url          = {http://joss.theoj.org/papers/10.21105/joss.00638}
}

@inproceedings{lugmayr2022repaint,
  title={Repaint: Inpainting using denoising diffusion probabilistic models},
  author={Lugmayr, Andreas and Danelljan, Martin and Romero, Andres and Yu, Fisher and Timofte, Radu and Van Gool, Luc},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11461--11471},
  year={2022}
}
@article{behrendt2023patched,
  title={Patched Diffusion Models for Unsupervised Anomaly Detection in Brain MRI},
  author={Behrendt, Finn and Bhattacharya, Debayan and Kr{\"u}ger, Julia and Opfer, Roland and Schlaefer, Alexander},
  journal={arXiv preprint arXiv:2303.03758},
  year={2023}
}
@article{ozdenizci2023restoring,
  title={Restoring vision in adverse weather conditions with patch-based denoising diffusion models},
  author={{\"O}zdenizci, Ozan and Legenstein, Robert},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2023},
  publisher={IEEE}
}


